Optimal Symbolic Bound Synthesis

The problem of finding a constant bound on a term given a set of assumptions has wide applications in optimization as well as program analysis. However, in many contexts the objective term may be unbounded. Still, some sort of symbolic bound may be useful. In this paper we introduce the optimal symbolic-bound synthesis problem, and a technique that tackles this problem for non-linear arithmetic with function symbols. This allows us to automatically produce symbolic bounds on complex arithmetic expressions from a set of both equality and inequality assumptions. Our solution employs a novel combination of powerful mathematical objects -- Gr\"obner bases together with polyhedral cones -- to represent an infinite set of implied inequalities. We obtain a sound symbolic bound by reducing the objective term by this infinite set. We implemented our method in a tool, AutoBound, which we tested on problems originating from real Solidity programs. We find that AutoBound yields relevant bounds in each case, matching or nearly-matching upper bounds produced by a human analyst on the same set of programs.

==> conclusion.tex <==
\section{Future Directions}
\label{Se:Conclusion}
In future work, we are interested in adopting our reduction techniques to more specific settings. For example, our polyhedron reduction algorithm works for conjunctive linear formulas. We suspect that a combination of polyhedral reduction with convex hull procedure could be used to give a complete and efficient solution to the OSB problem for arbitrary linear formulas. 
%In this context the convex hull is the analogue of our heuristic saturation step. In the case of convex hull a completeness argument can be made, which combined with our reduction algorithm would give a completeness result for linear formulas. However, the convex hull is often a very expensive method. We suspect that our polyhedral reduction algorithm could be combined with a convex hull procedure to yield a much more efficient method. 
%The idea is that our reduction method projects polyhedra down to a much smaller dimension, where convex hull operations become more feasible. 
Another possible future direction is the adaption of our techniques to the purely integer case. Our presentation considered polyhedra and ideals where the coefficients belong to a field. However, there are analogous, but much more expensive, polyhedra and Gr\"obner basis techniques that consider strictly integer coefficients. It would interesting to see if those methods could be adapted to the OSB problem while still being efficient.

==> theory.tex <==
\section{Theory}

\newcommand{\ThQ}{\mathcal{Q}}

\zak{Quick summary: I think that it is possible to formulate a theory such that the optimization problem is solvable.  However, it would require different techniques for handling axioms.  E.g., if we instantiate an axiom like $x = 1 \lor x = 2$, then we should be able to conclude $(x-1)(x-2) = 0$, but the convex hull algorithm will not discover this.  Furthermore, the theory can't really justify local projection [technical explanation: soundness of local projection relies on a total order.  We can extend $\leq_0$ to a total order, but not necessarily the others since the family of orders would effectively collapse and give us an "unbounded" product axiom].  So I don't know if this is an avenue worth pursuing.}


Let $\sigma_{\ThQ}$ be the signature containing two binary function symbols $+$ and $\cdot$, an infinite set of binary relation symbols $\{\leq_n\}_{n \in \mathbb{N}}$, each rational number as a constant symbol, and equality.
Consider the theory $\ThQ$ axiomatized by the following:

\[
\begin{array}{cr}
    \forall x,y,z. x+(y+z) = (x+y)+z \text{ and } \forall x,y,z. x \cdot (y \cdot z) = (x \cdot y) \cdot z & \text{(Associativity)}\\
    \forall x,y. x+y = y+x\text{ and  }\forall x,y. x\cdot y = y \cdot x & \text{(Commutativity)}\\
    \forall x. x+0 = x \text{ and } \forall x. x\cdot 1 = x & \text{(Identity)}\\
    \forall x. x + (-1) \cdot x = 0 & \text{(Inverse)}\\
    \forall x,y,z. x\cdot(y + z) = (x \cdot y) + (x \cdot z) & \text{(Distributivity)}\\
    \{\forall x. x \leq_n x\}_{n \in \mathbb{N}} & \text{(Reflexivity)}\\
    \{\forall x,y,z. x \leq_n y \land y \leq_n z \Rightarrow x \leq_n z\}_{n \in \mathbb{N}} & \text{(Transitivity)}\\
    \{\forall x,y,z. x \leq_n y \land y \leq_n x \Rightarrow x = y\}_{n \in \mathbb{N}} & \text{(Antisymmetry)}\\
    \{\forall x,y,z. (x \leq_n y \Rightarrow x + z \leq_n y + z)\}_{n \in \mathbb{N}} & \text{(Compatibility)}\\
    \{\forall x,y. (x \leq_n y \Rightarrow \lambda \cdot x \leq_n \lambda \cdot y)\}_{n \in \mathbb{N}, \lambda \in \mathbb{Q}^{\geq 0}}& \text{(Scaling)}\\
    \{\forall x,y. (0 \leq_{n+1} x \land 0 \leq_{n+1} y) \Rightarrow 0 \leq_{n} x\cdot y\}_{n \in \mathbb{N}} & \text{(Product)}\\
    \{\forall x,. x \leq_{n+1} y \Rightarrow x \leq_n y\}_{n \in \mathbb{N}} & \text{(Descent)}\\
    0 \neq 1 & \text{(Non-triviality})
\end{array} 
\]
as well as axioms defining the arithmetic of rationals
(for each triple of rationals $p,q,r$ such that $p + q = r$, we have the axioms $p + q = r$, similarly for multiplication and for $\leq_n$).\footnote{Note that this means that Inverse and Descent are redundant: 
$0 = (1 + -1)$, so $0 = 0x = (1 + -1)x = x + (-1)x$;
$0 \leq_{n+1} 1$, so for any $x$ with $0 \leq_{n+1} x$, we have $0 \leq_n 1x \equiv 0 \leq_n x$ by Product.}

Let $X$ be a set of constant symbols, and let $\mathfrak{A}$ a structure over a $\sigma_{\ThQ}$ extended with the symbols $X$ and which is a model of $\ThQ$. Observe that $\mathfrak{A}$ is a commutative ring containing a subring isomorphic to $\mathbb{Q}$.  For each $n \in \mathbb{N}$,
$\mathfrak{A}$ can be viewed as a partially ordered vector space over $\mathbb{Q}$ under the order $\leq_n$.  For any $n$, define \[C_n^\mathfrak{A} \defeq \{ p \in \mathbb{Q}[X] : \mathfrak{A} \models 0 \leq_n p \}\]
Observe that $C_n^\mathfrak{A}$ is a \textit{regular cone} (i.e., it is closed under addition, closed under multiplication by positive rationals, and its additive units form an ideal\footnote{Namely, the additive units of each $C_n^\mathfrak{A}$ is $\{ p \in \mathbb{Q}[X] : \mathfrak{A} \models 0 = p \}$}).  Furthermore the family $\{ C_n^\mathfrak{A}\}_{n \in \mathbb{N}}$ is \textbf{well-formed} in the sense that
\[ C_0^\mathfrak{A} \supseteq C_1^\mathfrak{A} \supseteq C_2^\mathfrak{A} \supseteq \dots \supseteq \mathbb{Q}^{\geq 0} \]
and for each $n$, $C_{n}^\mathfrak{A}$ contains $C_{n+1}^\mathfrak{A} \cdot C_{n+1}^\mathfrak{A} \defeq \{ p \cdot q : p,q \in C_{n+1} \}$, and the additive units of $C_0^\mathfrak{A}$ are the same as every other $C_i^{\mathfrak{A}}$.

In fact, any well-formed sequence of regular cones $\{C_n\}_{n \in \mathbb{Q}}$ such that $-1 \notin C_0$ defines a model $\mathfrak{C}$ of $\ThQ$:
\begin{itemize}
\item The universe $U^\mathfrak{C}$ is $\mathbb{Q}[X]/I = \{ p + I : p \in \mathbb{Q}[X] \}$, where $I$ is the ideal of additive units of $C_0$
\item $+^{\mathfrak{C}}$ and $\cdot^{\mathfrak{C}}$ are interpreted as in the ring $\mathbb{Q}[X]/I$
\item each constant symbol $k$ is interpreted as $k + I$
\item $\leq_n^\mathfrak{C} = \{ (p + I, q + I) : q-p \in C_n \}$
\end{itemize}

Let $P_0, P_1, \dots, P_k$ be a finite sequence of finite sets of polynomials over a set of variables $X$.  Then we can compute the smallest (w.r.t. inclusion order) well-formed family $\{ C_n \}_{n \in \mathbb{N}}$ such that $P_0 \subseteq C_0$, ..., $P_k \subseteq C_k$ by (1) using the saturation procedure to "regularize" each cone, and (2) using the product saturation procedure to enforce that each $C_n$ contains $C_{n+1} \cdot C_{n+1}$.  As a result, we can compute a "minimal model" of a conjunctive formula $F$:
let $k$ be the maximum natural such that $\leq_k$ appears in $F$, and for each $i \in \{0, ..., k\}$ define $P_i = \{ q-p : p \leq_i q \text{ occurs in } F\}$, and use the above algorithm to compute the smallest well-formed family of regular cones containing the $P_0,...,P_k$ sequence (i.e., $C_i$ contains $P_i$ for all $i$).  If $-1 \in C_0$, then the formula is inconsistent. Otherwise, we may define a model $\mathfrak{M}$ from the cone family as above.  We have that $\mathfrak{M}$ is minimal in the sense that
for any $n$, $\mathfrak{M} \models p \leq_n q$ if and only if $F \models p \leq_n q$ modulo $\ThQ$.  Applying the cone reduction procedure to $C_0$ gives us optimal upper bounds modulo the theory.

Extending with uninterpreted function symbols is straight-forward but technically a little tedious (since we need to work with a Herbrand universe instead of a set of polynomials)

\paragraph{Totality}

\begin{lemma}[Extension]
Let $X$ be a set of symbols, $C \subseteq \mathbb{Q}[X]$ be a regular cone, and let $p \in \mathbb{Q}[X]$ with $-p \notin C$.  Then $\{ q + \lambda p : q \in C, \lambda \in \mathbb{Q}^{\geq 0}\}$ is a regular cone, and has the same additive units as $C$.
\end{lemma}
\begin{proof}
Suppose that $r$ is an additive unit of $\{ q + \lambda p : q \in C, \lambda \in \mathbb{Q}^{\geq 0}\}$.  Then there is some $q_1,q_2 \in C$ and some $\lambda_1,\lambda_2 \in \mathbb{Q}^{\geq 0}$ such that $r = q_1 + \lambda_1 p$ and $-r = q_2 + \lambda_2 p$.  It follows that $0 = r - r = q_1+q_2 + (\lambda_1+\lambda_2)p$.  If $\lambda_1+\lambda_2$ is non-zero, then $-p = \frac{1}{\lambda_1+\lambda_2}(q_1+q_2) \in C$, contradicting our assumption that $-p \notin C$.  So $\lambda_1+\lambda_2$ must be zero, and thus both $\lambda_1$ and $\lambda_2$ are zero, and $r = q_1 \in C$.
\end{proof}

Suppose that we wish to extend the above theory with a totality axiom: $\forall x,y. x \leq_0 y \lor y \leq_0 x$.  The above procedure does \textit{not} compute models in the extended theory, because $C_0$ is not total (i.e., we do not have that for every $p$, either $p \in C_0$ or $-p \in C_0$); however, we can extend $C_0$ to make it total.
The idea is that we can simply enumerate all polynomials in $\mathbb{Q}[X]$ as $\{ p_i \}_{i \in \mathbb{N}}$ and construct a sequence of cones
\[C_{0,0} \subseteq C_{0,1} \subseteq \dotsi \]
where
\begin{align*}
 C_{0,0} &\defeq C_0\\
 C_{0,i+1} &\defeq \begin{cases} C_{0,i}  & \text{if } -p_{i} \in C_{0,i}\\
 \{ q + \lambda p_i : q \in C_{0,i}, \lambda \in \mathbb{Q}^{\geq 0}\} & \text{otherwise} \end{cases}
\end{align*}
and then take $C_0^{*} \defeq \bigcup_{i \in \mathbb{N}} C_{0,i}$.  By the extension lemma, each $C_{0,i}$ is a regular cone with the same additive units as $C_0$, so the same is true for $C_0^{*}$.  Constructing a model from this sequence (using $C_0^{*}$ in place of $C_0$) gives a model of the original theory, plus $\leq_0$ is total.

\paragraph{Inference rules}

\begin{mathpar}
\inferrule[Consistency]{
\varphi \vdash s_1 = t_1\\
\dots\\
\varphi \vdash s_n = t_n
}{
\varphi \vdash f(s_1,\dots,s_n) = f(t_1, \dots, t_n)
}

%\inferrule[(=)-Reflexivity]{
%}{
%\varphi \vdash t = t
%}

%\inferrule[(=)-Symmetry]{
%\varphi \vdash t = s
%}{
%\varphi \vdash s = t
%}

%\inferrule[(=)-Transitivity]{
%\varphi \vdash r = s\\
%\varphi \vdash s = t
%}{
%\varphi \vdash r = t
%}

%\inferrule[($\leq$)-Reflexivity]{
%}{
%\varphi \vdash t \leq_n t
%}

%\inferrule[($\leq$)-Antisymmetry]{
%\varphi \vdash s \leq_n t\\
%\varphi \vdash t \leq_n s
%}{
%\varphi \vdash s = t
%}

%\inferrule[($\leq$)-Transitivity]{
%\varphi \vdash r \leq_n s\\
%\varphi \vdash s \leq_n t
%}{
%\varphi \vdash r \leq_n t
%}

%\inferrule[($+$)-Commutativity]{
%}{
%\varphi \vdash s+t = t+s
%}

\inferrule[($*$)-Commutativity]{
}{
\varphi \vdash st = ts
}

%\inferrule[($+$)-Associativity]{
%}{
%\varphi \vdash r+(s+t) = (r+s)+t
%}

\inferrule[($*$)-Associativity]{
}{
\varphi \vdash r(st) = (rs)t
}

\inferrule[Distributivity]{
}{
\varphi \vdash (r+s)t = rt + st
}

%\inferrule[($+$)-Identity]{
%}{
%\varphi \vdash r + 0 = r
%}

\inferrule[($*$)-Identity]{
}{
\varphi \vdash r1 = r
}

%\inferrule[($+$)-Compatibility]{
%\varphi \vdash r \leq_n s
%}{
%\varphi \vdash r + t \leq_n s + t
%}

%\inferrule*[lab={Scaling},right={$\lambda \in %\mathbb{Q}^{\geq 0}$}]{
%\varphi \vdash r \leq_n s\\
%}{
%\varphi \vdash \lambda r \leq_n \lambda s
%}

\inferrule*[lab={Product},right={$i+j \leq n$}] {
  \varphi \vdash 0 \leq_i s\\
  \varphi \vdash 0 \leq_j t
}{
  \varphi \vdash 0 \leq_{i+j} st
}

\inferrule*[lab={Descent}] {
  \varphi \vdash s \leq_i t
}{
  \varphi \vdash s \leq_{i+1} t
}

\inferrule*[lab={LRA},right={$\varphi \land s_1 \leq t_1 \land \dots \land s_n \leq t_n \models_{LRA} s \leq t$}] {
  \varphi \vdash s_1 \leq_i t_1\\
  \dots\\
  \varphi \vdash s_n \leq_i t_n
}{
\varphi \vdash s \leq_i t
}
\end{mathpar}

In the above, $\models_{LRA}$ means entailment modulo the theory of Linear Real Arithmetic, in first order logic without equality (i.e., $=$ is an equivalence relation, but there is no functional consistency axiom).

(Equivalently, we might define the "product depth" of a derivation to be the maximum number of applications of the product rule on any path from the conclusion to a leaf, and then restrict our attention to derivations for product depth $\leq n$ for some $n$).

Given an input formula $\varphi$, the algorithm results in a rewrite system and (for each $i$) set of polynomials $P_\varphi(i)$.  For any term $t$, let  $\textbf{red}_\varphi(t)$ denote the normal form of $t$ w.r.t. the rewrite system.
\begin{conjecture}[Soundness]
  For each $i$ and each $p \in P_\varphi(i)$, we have $\varphi \vdash 0 \leq p$
\end{conjecture}
\begin{conjecture}[Completeness]
  If $\varphi \vdash s \leq_n t$ is derivable, then $\textbf{red}_\varphi(t-s)$ is a conic combination of the terms in $P_\varphi(i)$.  If $\varphi \vdash s = t$ is derivable, then
  $\textbf{red}_\varphi(t-s) = 0$.
\end{conjecture}

\begin{conjecture}[Optimality]
The optimization algorithm solves the following optimization problem:
\begin{quote}
    \textbf{Given} a quantifier-free formula $F$ and a term $t$, and a target set of constant symbols
    $W$, \textbf{find} a term $t^{*}$ such that
    \begin{enumerate}
    \item (Bound) $F \vdash t \leq_n t^{*}$
    \item (Optimality) For any term $s$ such that $F \vdash t \leq_n s$, we have $\effdegw{W}{t^{*}} \leq \effdegw{W}{s}$.
    \end{enumerate}
\end{quote}
\end{conjecture}
